Graph Neural Networks on Discriminative Graphs of Words

In light of the recent success of Graph Neural Networks (GNNs) and their ability to perform inference on complex data structures, many studies apply GNNs to the task of text classification. In most previous methods, a heterogeneous graph, containing both word and document nodes, is constructed using the entire corpus and a GNN is used to classify document nodes. In this work, we explore a new Discriminative Graph of Words Graph Neural Network (DGoW-GNN) approach encapsulating both a novel discriminative graph construction and model to classify text. In our graph construction, containing only word nodes and no document nodes, we split the training corpus into disconnected subgraphs according to their labels and weight edges by the pointwise mutual information of the represented words. Our graph construction, for which we provide theoretical motivation, allows us to reformulate the task of text classification as the task of walk classification. We also propose a new model for the graph-based classification of text, which combines a GNN and a sequence model. We evaluate our approach on seven benchmark datasets and find that it is outperformed by several state-of-the-art baseline models. We analyse reasons for this performance difference and hypothesise under which conditions it is likely to change.

==> Tables/Tabe_L1_nodes.tex <==
\begin{table}[]
\caption{The value of \textit{Adversarial Robustness} for our \textit{GCORN}, GCN and GCN-k. In this experiment, we set $p=1$ and $\epsilon=1.$}
\label{tab:prob_val_nodes}
% \resizebox{0.98\columnwidth}{!}{%
\centering
\begin{tabular}{lcccc}\toprule
       & \textbf{Cora}        & \textbf{CiteSeer}    & \textbf{PubMed}      & \textbf{CS}          \\ \toprule
\textbf{GCORN} & $ \mathbf{0.88 \pm 0.17}$ & $\mathbf{0.96 \pm 0.24}$ &$ \mathbf{1.49 \pm 0.25}$ & $\mathbf{0.09 \pm 0.05}$ \\
\textbf{GCN}    & $2.97 \pm 0.54$ & $2.93\pm  0.53$ & $2.79 \pm 0.60$ & $0.10 \pm 0.05$ \\
\textbf{GCN-k}  & $5.13 \pm 3.07$ & $7.23 \pm 1.14$ & $7.76 \pm 1.33$ & $ 0.46 (0.21) $ \\\toprule          
\end{tabular}

% }
\end{table}

==> Tables/Table_L1_Graphs.tex <==

\begin{table}[ht]
\centering

\caption{The value of \textit{Adversarial Robustness} for our \textit{RO-GCN}, GCN and GCN-k. In this experiment, we set $p=1$ and $\epsilon=1$}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{lcccc}\toprule
       & \textbf{DD}        & \textbf{NCI1}    & \textbf{PROTEINS}     \\ \toprule
\textbf{GCORN} & $ \mathbf{1.38 \pm 0.57 }$ & $\mathbf{10.07 \pm 2.68 }$ &$ \mathbf{3.14 \pm 0.68 }$  \\
\textbf{GCN}    & $1.46 \pm 0.41$ & $17.96 \pm 2.36 $ & $457 \pm 0.99 $ \\ \toprule          
\end{tabular}

}
\label{Tab:graph_adv}
\end{table}

==> Tables/node_classification_results.tex <==
% \setlength{\tabcolsep}{0.4em}
% \begin{table*}[h]
% %\tiny
% 	\centering
% 	\caption{Classification accuracy ($\pm$ standard deviation) of the models on different benchmark node classification dataset before (clean) and after the attack application. The higher the accuracy (in \%) the better the model. The best accuracy in each setting and each dataset is in \textbf{bold}.}
% 	\label{tab:results_node_classification}
%     \begin{tabular}{p{0.2\textwidth}cccccc}
%         \toprule
%         \multirow{Attack strategy} & \multicolumn{3}{c}{Cora} & \multicolumn{3}{c}{CiteSeer}\\
        
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
%         & \(\mathbf{GCN}\)  & \(\mathbf{GCN-k}\) & \(\mathbf{GCORN}\) & \(\mathbf{GCN}\) & \(\mathbf{GCN-k}\)  & \(\mathbf{GCORN}\)   \\
%         \midrule
%         Clean & \textbf{79.2 $\pm$ 1.6}   &  77.1 $\pm$ 1.4 & 78.8 $\pm$ 1.3 & 68.2 $\pm$ 1.2  & 68.1 $\pm$ 0.8 & \textbf{69.5 $\pm$ 1.1} \\
        
%         \hline
%         Random ($\psi = 0.5$) & 68.4 $\pm$ 1.9 & 69.2 $\pm$ 2.6 &  \textbf{77.1 $\pm$ 1.8} & 57.8 $\pm$ 1.5 & 62.3 $\pm$ 1.2 & \textbf{67.8 $\pm$ 1.4} \\
%         Random ($\psi = 1.0$) & 41.7 $\pm$ 2.1 & 46.3 $\pm$ 2.8 &  \textbf{57.6 $\pm$ 1.9} & 38.2 $\pm$ 1.3   & 45.3 $\pm$ 1.4 & \textbf{57.3 $\pm$ 1.7} \\
        
%         \hline
%         PGD ($\Delta = 0.15$) & 54.1 $\pm$ 2.4  & 58.3 $\pm$ 1.6 & \textbf{71.1 $\pm$ 1.4}  & 52.3 $\pm$ 1.1  & 59.6 $\pm$ 1.6  & \textbf{65.6 $\pm$ 1.4} \\
    
%         \toprule

%         \toprule
%         \multirow{Attack strategy} & \multicolumn{3}{c}{PubMed} & \multicolumn{3}{c}{CS}\\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
%         & \(\mathbf{GCN}\)  & \(\mathbf{GCN-k}\) & \(\mathbf{GCORN}\) & \(\mathbf{GCN}\)  & \(\mathbf{GCN-k}\) & \(\mathbf{GCORN}\)    \\
%         \midrule
%         Clean & \textbf{76.3 $\pm$ 0.7} & 74.7 $\pm$ 0.8 & 75.6 $\pm$ 1.4  & \textbf{92.9 $\pm$ 0.5}  & 92.6 $\pm$ 0.3 & 91.5 $\pm$ 0.8\\
        
%         \hline
%         Random ($\psi = 0.5$) & 68.5 $\pm$ 1.2   & 71.2 $\pm$ 1.1 & \textbf{73.1 $\pm$ 1.1} &  85.3 $\pm$ 1.1  & 86.7 $\pm$ 1.1 & \textbf{89.8 $\pm$ 1.2} \\
%         Random ($\psi = 1.0$) & 60.1 $\pm$ 1.7  & 62.3 $\pm$ 1.3 & \textbf{65.8 $\pm$ 1.4} & 69.9 $\pm$ 1.3   & 73.2 $\pm$ 0.9 & \textbf{81.3 $\pm$ 1.6}\\
        
%         \hline
%         PGD ($\Delta = 0.15$) & 66.1 $\pm$ 2.4 & 67.3 $\pm$ 1.6 & \textbf{71.1 $\pm$ 1.4}  & 71.3 $\pm$ 1.1 & 74.1 $\pm$ 0.8 & \textbf{79.6 $\pm$ 1.2}\\
    
%         \toprule
        
        
%         \end{tabular}

% \end{table*}

% \setlength{\tabcolsep}{0.2em}

% \begin{table*}[h]
% %\tiny
% 	\centering
% 	\caption{Classification accuracy ($\pm$ standard deviation) of the models on different benchmark node classification dataset before (clean) and after the attack application. The higher the accuracy (in \%) the better the model. The best accuracy in each setting and each dataset is in \textbf{bold}.}
% 	\label{tab:results_node_classification}
%     \begin{tabular}{p{0.09\textwidth}cccccccc}
%         \toprule %strategy
%         \multirow{Attack} & \multicolumn{4}{c}{Cora} & \multicolumn{4}{c}{CiteSeer}\\
        
%         \cmidrule(lr){2-5} \cmidrule(lr){6-9} 
%         & \(\mathbf{GCN}\)  & \(\mathbf{GCN-k}\) & \(\mathbf{RGCN}\) & \(\mathbf{GCORN}\) & \(\mathbf{GCN}\) & \(\mathbf{GCN-k}\) & \(\mathbf{RGCN}\)  & \(\mathbf{GCORN}\)   \\
%         \midrule
%         Clean & \textbf{79.2$\pm$1.6}  & 77.1$\pm$1.4 & 79.1$\pm$0.4  & 78.8$\pm$1.3 & 68.2$\pm$1.2  & 68.1$\pm$0.8 & 68.9$\pm$0.5 & \textbf{69.5$\pm$1.1} \\
        
%         \hline %($\psi = 0.5$) ($\psi = 1.0$) ($\Delta = 0.15$)
%         Random  & 68.4$\pm$1.9 & 69.2$\pm$2.6 & 70.6$\pm$0.3 &  \textbf{77.1$\pm$1.8} & 57.8$\pm$1.5 & 62.3$\pm$1.2 & 63.7$\pm$0.6 & \textbf{67.8$\pm$1.4} \\
        
%         Random & 41.7$\pm$2.1 & 46.3$\pm$2.8 & 52.8$\pm$1.6 &  \textbf{57.6$\pm$1.9} & 38.2$\pm$1.3   & 45.3$\pm$1.4 & 43.7$\pm$2.2 & \textbf{57.3$\pm$1.7} \\
        
%         \hline
%         PGD & 54.1$\pm$2.4  & 58.3$\pm$1.6 & 62.5$\pm$1.2 & \textbf{71.1$\pm$1.4}  & 52.3$\pm$1.1  & 59.6$\pm$1.6 & 61.9$\pm$1.1 & \textbf{65.6$\pm$1.4} \\
    
%         Nettack & 60.9$\pm$2.5  & 64.2$\pm$5.2 & 63.4$\pm$3.8 & \textbf{68.3$\pm$1.4}  & 55.8$\pm$1.4  & 71.7$\pm$1.4 & 70.8$\pm$3.8 & \textbf{77.5$\pm$2.5} \\
    
%         \toprule

%         \toprule
%         \multirow{Attack} & \multicolumn{4}{c}{PubMed} & \multicolumn{4}{c}{CS}\\
%         \cmidrule(lr){2-5} \cmidrule(lr){6-9} 
%         & \(\mathbf{GCN}\)  & \(\mathbf{GCN-k}\) & \(\mathbf{RGCN}\) & \(\mathbf{GCORN}\) & \(\mathbf{GCN}\) & \(\mathbf{GCN-k}\) & \(\mathbf{RGCN}\)  & \(\mathbf{GCORN}\)   \\
%         \midrule
    
%         Clean & 76.3$\pm$0.7 & 74.7$\pm$0.8 & \textbf{76.6$\pm$0.6} & 76.1$\pm$1.4  & \textbf{92.9$\pm$0.5}  & 92.6$\pm$0.3 & 91.2$\pm$0.7 & 91.5$\pm$0.8\\
        
%         \hline
%         Random  & 68.5$\pm$1.2   & 71.2$\pm$1.1 & 70.0$\pm$0.5 & \textbf{73.1$\pm$1.1} &  85.3$\pm$1.1  & 86.7$\pm$1.1 & 88.2$\pm$0.9   & \textbf{89.8$\pm$1.2} \\
%         Random  & 60.1$\pm$1.7  & 62.3$\pm$1.3 & 61.9$\pm$1.2 & \textbf{65.8$\pm$1.4} & 69.9$\pm$1.3   & 73.2$\pm$0.9 & 76.2$\pm$1.4 & \textbf{81.3$\pm$1.6}\\
        
%         \hline
%         PGD  & 66.1$\pm$2.4 & 67.3$\pm$1.6 & 69.5$\pm$0.9 & \textbf{71.1$\pm$1.4}  & 71.3$\pm$1.1 & 74.1$\pm$0.8 & 76.6$\pm$1.2 & \textbf{79.6$\pm$1.2}\\

%         Nettack  & 60.0$\pm$2.5 & 65.8$\pm$2.9 & \textbf{71.7$\pm$3.8} & 70.8$\pm$1.4  & 55.8$\pm$1.4 & 71.6$\pm$1.4 & 71.7$\pm$2.9 & \textbf{78.3$\pm$1.4}\\

        
%         \toprule
        
        
%         \end{tabular}

% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
% \centering

% \caption{Classification accuracy ($\pm$ standard deviation) of the models on different benchmark node classification dataset before (clean) and after the attack application. The higher the accuracy (in \%) the better the model. The best accuracy in each setting and each dataset is in \textbf{bold}.}
% \label{tab:results_node_classification}


% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \multirow{2}{*}{Attack} & \multicolumn{4}{c}{Cora}                                                            & \multicolumn{4}{c}{CiteSeer}                                               \\ \cmidrule(l){2-9} 
%                         & \textbf{GCN}            & \textbf{GCN-k} & \textbf{RGCN}  & \textbf{GCORN}          & \textbf{GCN}   & \textbf{GCN-k} & \textbf{RGCN}  & \textbf{GCORN}          \\ \midrule
% Clean                   & \textbf{79.2 $\pm$ 1.6} & 77.1 $\pm$ 1.4 & 79.1 $\pm$ 0.4 & 78.8 $\pm$ 1.3          & 68.2 $\pm$ 1.2 & 68.1 $\pm$ 0.8 & 68.9 $\pm$ 0.5 & \textbf{69.5 $\pm$ 1.1} \\ \midrule
% Random ($\psi = 0.5$)  & 68.4 $\pm$ 1.9          & 69.2 $\pm$ 2.6 & 70.6 $\pm$ 0.3 & \textbf{77.1 $\pm$ 1.8} & 57.8 $\pm$ 1.5 & 62.3 $\pm$ 1.2 & 63.7 $\pm$ 0.6 & \textbf{67.8 $\pm$ 1.4} \\
% Random ($\psi = 1.0$)  & 41.7 $\pm$ 2.1          & 46.3 $\pm$ 2.8 & 52.8 $\pm$ 1.6 & \textbf{57.6 $\pm$ 1.9} & 38.2 $\pm$ 1.3 & 45.3 $\pm$ 1.4 & 43.7 $\pm$ 2.2 & \textbf{57.3 $\pm$ 1.7} \\ \midrule
% PGD                     & 54.1 $\pm$ 2.4          & 58.3 $\pm$ 1.6 & 62.5 $\pm$ 1.2 & \textbf{71.1 $\pm$ 1.4} & 52.3 $\pm$ 1.1 & 59.6 $\pm$ 1.6 & 61.9 $\pm$ 1.1 & \textbf{65.6 $\pm$ 1.4} \\
% Nettack                 & 60.9 $\pm$ 2.5          & 64.2 $\pm$ 5.2 & 63.4 $\pm$ 3.8 & \textbf{68.3 $\pm$ 1.4} & 55.8 $\pm$ 1.4 & 71.7 $\pm$ 1.4 & 70.8 $\pm$ 3.8 & \textbf{77.5 $\pm$ 2.5} \\ \bottomrule

% \toprule

% \toprule


% \multirow{2}{*}{Attack} & \multicolumn{4}{c}{PubMed}                                                                   & \multicolumn{4}{c}{CS}                                                     \\ \cmidrule(l){2-9} 
%                         & \textbf{GCN}            & \textbf{GCN-k} & \textbf{RGCN}           & \textbf{GCORN}          & \textbf{GCN}   & \textbf{GCN-k} & \textbf{RGCN}  & \textbf{GCORN}          \\ \midrule
% Clean                   & \textbf{76.3 $\pm$ 0.7} & 74.7 $\pm$ 0.8 & \textbf{76.6 $\pm$ 0.6} & 76.1 $\pm$ 1.4          & 92.9 $\pm$ 0.5 & 92.6 $\pm$ 0.3 & 91.2 $\pm$ 0.7 & \textbf{91.5 $\pm$ 0.8} \\ \midrule
% Random ($\psi = 0.5$)  & 68.3 $\pm$ 1.2          & 71.2 $\pm$ 1.1 & 71.4 $\pm$ 0.5          & \textbf{73.1 $\pm$ 1.1} & 85.3 $\pm$ 1.1 & 86.7 $\pm$ 1.1 & 88.2 $\pm$ 0.9 & \textbf{89.8 $\pm$ 1.2} \\
% Random ($\psi = 1.0$)  & 60.1 $\pm$ 1.7          & 62.3 $\pm$ 1.3 & 61.9 $\pm$ 1.2          & \textbf{65.8 $\pm$ 1.4} & 69.9 $\pm$ 1.3 & 73.2 $\pm$ 0.9 & 76.2 $\pm$ 1.4 & \textbf{81.3 $\pm$ 1.6} \\ \midrule
% PGD                     & 66.1 $\pm$ 2.1          & 67.3 $\pm$ 1.3 & 69.5 $\pm$ 0.9          & \textbf{72.3 $\pm$ 1.3} & 71.3 $\pm$ 1.1 & 74.1 $\pm$ 0.8 & 76.6 $\pm$ 1.2 & \textbf{79.6 $\pm$ 1.2} \\
% Nettack                 & 60.0 $\pm$ 2.5          & 65.8 $\pm$ 2.9 & \textbf{71.7 $\pm$ 3.8} & 70.8 $\pm$ 1.4          & 55.8 $\pm$ 1.4 & 71.6 $\pm$ 1.4 & 71.7 $\pm$ 2.9 & \textbf{78.3 $\pm$ 1.4} \\ \bottomrule
% \end{tabular}%

% }

% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[t]

% \centering

% \caption{Classification accuracy ($\pm$ standard deviation) of the models on different benchmark node classification dataset before (``Clean'') and after the attack application. The higher the accuracy (in \%) the better the model. The best accuracy in each setting and each dataset is typeset in \textbf{bold}.}
% \label{tab:results_node_classification}


% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lcccccccccc@{}}
% \toprule
% \multirow{2}{*}{} & \multicolumn{5}{c}{Cora}                                                                                                  & \multicolumn{5}{c}{CiteSeer}                                                                 \\ \cmidrule(l){2-11} 
%                         & \textbf{GCN}   & \textbf{GCN-k} & \textbf{AirGNN}         & \textbf{RGCN}           & \multicolumn{1}{c|}{\textbf{GCORN}}          & \textbf{GCN}            & \textbf{GCN-k} & \textbf{AirGNN} & \textbf{RGCN}  & \textbf{GCORN}          \\ \midrule
% Clean                   & 79.2 $\pm$ 1.6 & 77.1 $\pm$ 1.4 & \textbf{79.8 $\pm$ 0.5} & 79.1 $\pm$ 0.4          & \multicolumn{1}{c|}{78.8 $\pm$ 1.3}          & 68.2 $\pm$ 1.2          & 68.1 $\pm$ 0.8 & 67.8 $\pm$ 0.8  & 68.9 $\pm$ 0.5 & \textbf{69.5 $\pm$ 1.1} \\ \midrule
% Random ($\psi = 0.5$)  & 68.4 $\pm$ 1.9 & 69.2 $\pm$ 2.6 & 68.5 $\pm$ 1.9          & 70.6 $\pm$ 0.3          & \multicolumn{1}{c|}{\textbf{77.1 $\pm$ 1.8}} & 57.8 $\pm$ 1.5          & 62.3 $\pm$ 1.2 & 52.6 $\pm$ 1.6  & 63.7 $\pm$ 0.6 & \textbf{67.8 $\pm$ 1.4} \\
% Random ($\psi = 1.0$)  & 41.7 $\pm$ 2.1 & 46.3 $\pm$ 2.8 & 47.7 $\pm$ 2.2          & 52.8 $\pm$ 1.6          & \multicolumn{1}{c|}{\textbf{57.6 $\pm$ 1.9}} & 38.2 $\pm$ 1.3          & 45.3 $\pm$ 1.4 & 41.4 $\pm$ 2.5  & 43.7 $\pm$ 2.2 & \textbf{57.3 $\pm$ 1.7} \\ \midrule
% PGD                     & 54.1 $\pm$ 2.4 & 58.3 $\pm$ 1.6 & 68.2 $\pm$ 1.8          & 62.5 $\pm$ 1.2          & \multicolumn{1}{c|}{\textbf{71.1 $\pm$ 1.4}} & 52.3 $\pm$ 1.1          & 59.6 $\pm$ 1.6 & 56.3 $\pm$ 2.1  & 61.9 $\pm$ 1.1 & \textbf{65.6 $\pm$ 1.4} \\
% Nettack                 & 60.9 $\pm$ 2.5 & 64.2 $\pm$ 5.2 &  66.7 $\pm$ 3.8   & 63.4 $\pm$ 3.8          & \multicolumn{1}{c|}{\textbf{68.3 $\pm$ 1.4}} & 55.8 $\pm$ 1.4          & 71.7 $\pm$ 1.4 &  67.5 $\pm$ 2.5               & 70.8 $\pm$ 3.8 & \textbf{77.5 $\pm$ 2.5} \\ 

% \toprule

% \toprule

% \multirow{2}{*}{} & \multicolumn{5}{c}{PubMed}                                                                                                & \multicolumn{5}{c}{CS}                                                                       \\ \cmidrule(l){2-11} 
%                         & \textbf{GCN}   & \textbf{GCN-k} & \textbf{AirGNN}         & \textbf{RGCN}           & \multicolumn{1}{c|}{\textbf{GCORN}}          & \textbf{GCN}            & \textbf{GCN-k} & \textbf{AirGNN} & \textbf{RGCN}  & \textbf{GCORN}          \\ \midrule
% Clean                   & 76.3 $\pm$ 0.7 & 74.7 $\pm$ 0.8 & 76.4 + 0.2              & \textbf{76.6 $\pm$ 0.6} & \multicolumn{1}{c|}{76.1 $\pm$ 1.4}          & \textbf{92.9 $\pm$ 0.5} & 92.6 $\pm$ 0.3 & 90.8 $\pm$ 0.9  & 91.2 $\pm$ 0.7 & 91.5 $\pm$ 0.8          \\ \midrule
% Random ($\psi = 0.5$)  & 68.3 $\pm$ 1.2 & 71.2 $\pm$ 1.1 & 66.9 $\pm$ 1.3          & 71.4 $\pm$ 0.5          & \multicolumn{1}{c|}{\textbf{73.1 $\pm$ 1.1}} & 85.3 $\pm$ 1.1          & 86.7 $\pm$ 1.1 & 87.5 $\pm$ 1.6  & 88.2 $\pm$ 0.9 & \textbf{89.8 $\pm$ 1.2} \\
% Random ($\psi = 1.0$)  & 60.1 $\pm$ 1.7 & 62.3 $\pm$ 1.3 & 62.4 $\pm$ 1.2          & 61.9 $\pm$ 1.2          & \multicolumn{1}{c|}{\textbf{65.8 $\pm$ 1.4}} & 69.9 $\pm$ 1.3          & 73.2 $\pm$ 0.9 & 73.7 $\pm$ 2.8  & 76.2 $\pm$ 1.4 & \textbf{81.3 $\pm$ 1.6} \\ \midrule
% PGD                     & 66.1 $\pm$ 2.1 & 67.3 $\pm$ 1.3 & 70.8 $\pm$ 1.7          & 69.5 $\pm$ 0.9          & \multicolumn{1}{c|}{\textbf{72.3 $\pm$ 1.3}} & 71.3 $\pm$ 1.1          & 74.1 $\pm$ 0.8 & 76.3 $\pm$ 2.1  & 76.6 $\pm$ 1.2 & \textbf{79.6 $\pm$ 1.2} \\
% Nettack                 & 60.0 $\pm$ 2.5 & 65.8 $\pm$ 2.9 & 69.2 $\pm$ 1.4   & \textbf{71.7 $\pm$ 3.8} & \multicolumn{1}{c|}{70.8 $\pm$ 1.4}          & 55.8 $\pm$ 1.4          & 71.6 $\pm$ 1.4 & 76.7 $\pm$ 1.4    & 71.7 $\pm$ 2.9 & \textbf{78.3 $\pm$ 1.4} \\ \bottomrule
% \end{tabular}%
% }
% \end{table}


% \begin{table}[t]

% \centering

% \caption{Classification accuracy ($\pm$ standard deviation) of the models on different benchmark node classification dataset before (``Clean'') and after the attack application. The higher the accuracy (in \%) the better the model. The best accuracy in each setting and each dataset is typeset in \textbf{bold}.}
% \label{tab:results_node_classification}


% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lcccccccccc@{}}
% \toprule
% \multirow{2}{*}{} & \multicolumn{5}{c}{Cora}                                                                                                  & \multicolumn{5}{c}{CiteSeer}                                                                 \\ \cmidrule(l){2-11} 
%                         & \textbf{GCN}   & \textbf{GCN-k} & \textbf{AirGNN}         & \textbf{RGCN}           & \multicolumn{1}{c|}{\textbf{GCORN}}          & \textbf{GCN}            & \textbf{GCN-k} & \textbf{AirGNN} & \textbf{RGCN}  & \textbf{GCORN}          \\ \midrule
% Clean                   & 79.2 $\pm$ 1.6 & 77.1 $\pm$ 1.4 & \textbf{79.8 $\pm$ 0.5} & 79.1 $\pm$ 0.4          & \multicolumn{1}{c|}{78.8 $\pm$ 1.3}          & 68.2 $\pm$ 1.2          & 68.1 $\pm$ 0.8 & 67.8 $\pm$ 0.8  & 68.9 $\pm$ 0.5 & \textbf{69.5 $\pm$ 1.1} \\ \midrule
% Random ($\psi = 0.5$)  & 68.4 $\pm$ 1.9 & 69.2 $\pm$ 2.6 & 68.5 $\pm$ 1.9          & 70.6 $\pm$ 0.3          & \multicolumn{1}{c|}{\textbf{77.1 $\pm$ 1.8}} & 57.8 $\pm$ 1.5          & 62.3 $\pm$ 1.2 & 52.6 $\pm$ 1.6  & 63.7 $\pm$ 0.6 & \textbf{67.8 $\pm$ 1.4} \\
% Random ($\psi = 1.0$)  & 41.7 $\pm$ 2.1 & 46.3 $\pm$ 2.8 & 47.7 $\pm$ 2.2          & 52.8 $\pm$ 1.6          & \multicolumn{1}{c|}{\textbf{57.6 $\pm$ 1.9}} & 38.2 $\pm$ 1.3          & 45.3 $\pm$ 1.4 & 41.4 $\pm$ 2.5  & 43.7 $\pm$ 2.2 & \textbf{57.3 $\pm$ 1.7} \\ \midrule
% PGD                     & 54.1 $\pm$ 2.4 & 58.3 $\pm$ 1.6 & 68.2 $\pm$ 1.8          & 62.5 $\pm$ 1.2          & \multicolumn{1}{c|}{\textbf{71.1 $\pm$ 1.4}} & 52.3 $\pm$ 1.1          & 59.6 $\pm$ 1.6 & 56.3 $\pm$ 2.1  & 61.9 $\pm$ 1.1 & \textbf{65.6 $\pm$ 1.4} \\
% Nettack                 & 60.9 $\pm$ 2.5 & 64.2 $\pm$ 5.2 &  66.7 $\pm$ 3.8   & 63.4 $\pm$ 3.8          & \multicolumn{1}{c|}{\textbf{68.3 $\pm$ 1.4}} & 55.8 $\pm$ 1.4          & 71.7 $\pm$ 1.4 &  67.5 $\pm$ 2.5               & 70.8 $\pm$ 3.8 & \textbf{77.5 $\pm$ 2.5} \\ 

% \toprule

% \toprule

% \multirow{2}{*}{} & \multicolumn{5}{c}{PubMed}                                                                                                & \multicolumn{5}{c}{CS}                                                                       \\ \cmidrule(l){2-11} 
%                         & \textbf{GCN}   & \textbf{GCN-k} & \textbf{AirGNN}         & \textbf{RGCN}           & \multicolumn{1}{c|}{\textbf{GCORN}}          & \textbf{GCN}            & \textbf{GCN-k} & \textbf{AirGNN} & \textbf{RGCN}  & \textbf{GCORN}          \\ \midrule
% Clean                   & 76.3 $\pm$ 0.7 & 74.7 $\pm$ 0.8 & 76.4 + 0.2              & \textbf{76.6 $\pm$ 0.6} & \multicolumn{1}{c|}{76.1 $\pm$ 1.4}          & \textbf{92.9 $\pm$ 0.5} & 92.6 $\pm$ 0.3 & 90.8 $\pm$ 0.9  & 91.2 $\pm$ 0.7 & 91.5 $\pm$ 0.8          \\ \midrule
% Random ($\psi = 0.5$)  & 68.3 $\pm$ 1.2 & 71.2 $\pm$ 1.1 & 66.9 $\pm$ 1.3          & 71.4 $\pm$ 0.5          & \multicolumn{1}{c|}{\textbf{73.1 $\pm$ 1.1}} & 85.3 $\pm$ 1.1          & 86.7 $\pm$ 1.1 & 87.5 $\pm$ 1.6  & 88.2 $\pm$ 0.9 & \textbf{89.8 $\pm$ 1.2} \\
% Random ($\psi = 1.0$)  & 60.1 $\pm$ 1.7 & 62.3 $\pm$ 1.3 & 62.4 $\pm$ 1.2          & 61.9 $\pm$ 1.2          & \multicolumn{1}{c|}{\textbf{65.8 $\pm$ 1.4}} & 69.9 $\pm$ 1.3          & 73.2 $\pm$ 0.9 & 73.7 $\pm$ 2.8  & 76.2 $\pm$ 1.4 & \textbf{81.3 $\pm$ 1.6} \\ \midrule
% PGD                     & 66.1 $\pm$ 2.1 & 67.3 $\pm$ 1.3 & 70.8 $\pm$ 1.7          & 69.5 $\pm$ 0.9          & \multicolumn{1}{c|}{\textbf{72.3 $\pm$ 1.3}} & 71.3 $\pm$ 1.1          & 74.1 $\pm$ 0.8 & 76.3 $\pm$ 2.1  & 76.6 $\pm$ 1.2 & \textbf{79.6 $\pm$ 1.2} \\
% Nettack                 & 60.0 $\pm$ 2.5 & 65.8 $\pm$ 2.9 & 69.2 $\pm$ 1.4   & \textbf{71.7 $\pm$ 3.8} & \multicolumn{1}{c|}{70.8 $\pm$ 1.4}          & 55.8 $\pm$ 1.4          & 71.6 $\pm$ 1.4 & 76.7 $\pm$ 1.4    & 71.7 $\pm$ 2.9 & \textbf{78.3 $\pm$ 1.4} \\ 


% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}

\begin{table}[t]

\centering

\caption{Classification accuracy ($\pm$ standard deviation) of the models on different benchmark node classification dataset before (``Clean'') and after the attack application. The higher the accuracy (in \%) the better the model. The best accuracy in each setting and each dataset is typeset in \textbf{bold}.}
\label{tab:results_node_classification}


\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\multirow{2}{*}{Attack} & \multicolumn{5}{c}{Cora}                                                                                                  & \multicolumn{5}{c}{CS}                                                                                    \\ \cmidrule(l){2-11} 
                        & \textbf{GCN}   & \textbf{GCN-k} & \textbf{AirGNN}         & \textbf{RGCN}           & \multicolumn{1}{c|}{\textbf{GCORN}}          & \textbf{GCN}            & \textbf{GCN-k} & \textbf{AirGNN}             & \textbf{RGCN}  & \textbf{GCORN}           \\ \midrule
Clean                   & 79.2 $\pm$ 1.6 & 77.1 $\pm$ 1.4 & \textbf{79.8 $\pm$ 0.5} & 79.1 $\pm$ 0.4          & \multicolumn{1}{c|}{78.8 $\pm$ 1.3}          & \textbf{92.9 $\pm$ 0.5} & 92.6 $\pm$ 0.3 & 90.8 $\pm$ 0.9              & 91.2 $\pm$ 0.7 & 91.5 $\pm$ 0.8  \\ \midrule
Random ($\psi = 0.5$)  & 68.4 $\pm$ 1.9 & 69.2 $\pm$ 2.6 & 68.5 $\pm$ 1.9          & 70.6 $\pm$ 0.3          & \multicolumn{1}{c|}{\textbf{77.1 $\pm$ 1.8}} & 85.3 $\pm$ 1.1          & 86.7 $\pm$ 1.1 & 87.5 $\pm$ 1.6              & 88.2 $\pm$ 0.9 & \textbf{89.8 $\pm$ 1.2}  \\
Random ($\psi = 1.0$)  & 41.7 $\pm$ 2.1 & 46.3 $\pm$ 2.8 & 47.7 $\pm$ 2.2          & 52.8 $\pm$ 1.6          & \multicolumn{1}{c|}{\textbf{57.6 $\pm$ 1.9}} & 69.9 $\pm$ 1.3          & 73.2 $\pm$ 0.9 & 73.7 $\pm$ 2.8              & 76.2 $\pm$ 1.4 & \textbf{81.3 $\pm$ 1.6}  \\ \midrule
PGD                     & 54.1 $\pm$ 2.4 & 58.3 $\pm$ 1.6 & 68.2 $\pm$ 1.8          & 62.5 $\pm$ 1.2          & \multicolumn{1}{c|}{\textbf{71.1 $\pm$ 1.4}} & 71.3 $\pm$ 1.1          & 74.1 $\pm$ 0.8 & 76.3 $\pm$ 2.1              & 76.6 $\pm$ 1.2 & \textbf{79.6 $\pm$ 1.2}  \\
Nettack                 & 60.9 $\pm$ 2.5 & 64.2 $\pm$ 5.2 & 66.7 $\pm$ 3.8          & 63.4 $\pm$ 3.8          & \multicolumn{1}{c|}{\textbf{68.3 $\pm$ 1.4}} & 55.8 $\pm$ 1.4          & 71.6 $\pm$ 1.4 & 76.7 $\pm$ 1.4 & 71.7 $\pm$ 2.9 & \textbf{78.3 $\pm$ 1.4}  \\ \midrule
\multirow{2}{*}{Attack} & \multicolumn{5}{c}{PubMed}                                                                                                & \multicolumn{5}{c}{OGBN-Arxiv}                                                                            \\ \cmidrule(l){2-11} 
                        & \textbf{GCN}   & \textbf{GCN-k} & \textbf{AirGNN}         & \textbf{RGCN}           & \multicolumn{1}{c|}{\textbf{GCORN}}          & \textbf{GCN}            & \textbf{GCN-k} & \textbf{AirGNN}             & \textbf{RGCN}  & \textbf{GCORN}           \\ \midrule
Clean                   & 76.3 $\pm$ 0.7 & 74.7 $\pm$ 0.8 & 76.4 + 0.2              & \textbf{76.6 $\pm$ 0.6} & \multicolumn{1}{c|}{76.1 $\pm$ 1.4}          & 68.9 $\pm$ 0.7          & 56.0 $\pm$ 0.3 & 61.9 $\pm$ 0.9              & 65.1 $\pm$ 1.8 & \textbf{69.6 $\pm$ 1.2}  \\ \midrule
Random ($\psi = 0.5$)  & 68.3 $\pm$ 1.2 & 71.2 $\pm$ 1.1 & 66.9 $\pm$ 1.3          & 71.4 $\pm$ 0.5          & \multicolumn{1}{c|}{\textbf{73.1 $\pm$ 1.1}} & 68.2 $\pm$ 1.5          & 52.8 $\pm$ 0.5 & 59.0 $\pm$ 1.3              & 63.8 $\pm$ 1.9 & \textbf{69.1 $\pm$ 1.8}  \\
Random ($\psi = 1.0$)  & 60.1 $\pm$ 1.7 & 62.3 $\pm$ 1.3 & 62.4 $\pm$ 1.2          & 61.9 $\pm$ 1.2          & \multicolumn{1}{c|}{\textbf{65.8 $\pm$ 1.4}} & 66.4 $\pm$ 1.9          & 46.6 $\pm$ 0.6 & 51.9 $\pm$ 1.6              & 63.0 $\pm$ 2.4 & \textbf{67.3  $\pm$ 2.1} \\ \midrule
PGD                     & 66.1 $\pm$ 2.1 & 67.3 $\pm$ 1.3 & 70.8 $\pm$ 1.7          & 69.5 $\pm$ 0.9          & \multicolumn{1}{c|}{\textbf{72.3 $\pm$ 1.3}} & 67.5 $\pm$ 0.9          & 49.9 $\pm$ 0.7 & 55.7 $\pm$ 0.9              & 63.6 $\pm$ 0.7 & \textbf{68.1 $\pm$ 1.1}  \\
Nettack                 & 60.0 $\pm$ 2.5 & 65.8 $\pm$ 2.9 & 69.2 $\pm$ 1.4          & \textbf{71.7 $\pm$ 3.8} & \multicolumn{1}{c|}{70.8 $\pm$ 1.4}          & 49.2 $\pm$ 2.9          & 53.3 $\pm$ 1.4 & \textbf{56.7 $\pm$ 1.4}     & 52.6 $\pm$ 2.5 & 55.8 $\pm$ 1.4           \\ \bottomrule
\end{tabular}%
}
\end{table}

==> Tables/robustness_evaluation.tex <==

\begin{table*}[ht]

	\centering
	\caption{Classification accuracy ($\pm$ standard deviation) of the models on different benchmark graph classification dataset before (clean) and after the attack application. The higher the accuracy (in \%) the better the model.}
	\label{tab:results_node_classification}
    \begin{tabular}{p{0.25\textwidth}cccccc}
        \toprule
        \multirow{Attack strategy} & \multicolumn{3}{c}{Cora} & \multicolumn{3}{c}{CiteSeer}\\
        
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
        & \(\mathbf{GCN}\)  & \(\mathbf{RO-GCN}\) & \(\mathbf{GCN-k}\) & \(\mathbf{GCN}\)  & \(\mathbf{RO-GCN}\) & \(\mathbf{GCN-k}\)    \\
        \midrule
        Clean & 79.2 $\pm$ 1.6   & 78.8 $\pm$ 1.3  &  77.1 $\pm$ 1.4 & 68.2 $\pm$ 1.2  & 69.5 $\pm$ 1.1 & 68.1 $\pm$ 0.8 \\
        
        \hline
        Random attack ($\beta = 0.5$) & 68.4 $\pm$ 1.9 &  77.1 $\pm$ 1.8 & 69.2 $\pm$ 2.6 & 57.8 $\pm$ 1.5 & 67.8 $\pm$ 1.4 & 62.3 $\pm$ 1.2 \\
        Random attack ($\beta = 1.0$) & 41.7 $\pm$ 2.1 &  57.6 $\pm$ 1.9 & 46.3 $\pm$ 2.8 & 38.2 $\pm$ 1.3  & 57.3 $\pm$ 1.7 & 45.3 $\pm$ 1.4 \\
        
        \hline
        Gradient-based ($\Delta = 0.15$) & 54.1 $\pm$ 2.4 & 71.1 $\pm$ 1.4 & 58.3 $\pm$ 1.6  & 52.3 $\pm$ 1.1  & 65.6 $\pm$ 1.4 & 59.6 $\pm$ 1.6 \\
    
        \toprule


        \toprule
        \multirow{Attack strategy} & \multicolumn{3}{c}{PubMed} & \multicolumn{3}{c}{CS}\\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
        & \(\mathbf{GCN}\)  & \(\mathbf{RO-GCN}\) & \(\mathbf{RO-GCN}\) & \(\mathbf{GCN}\)  & \(\mathbf{RO-GCN}\) & \(\mathbf{GCN-k}\)    \\
        \midrule
        Clean & 76.3 $\pm$ 0.7   & 75.6 $\pm$ 1.4  & 74.7 $\pm$ 0.8  & 92.9 $\pm$ 0.5 & 91.5 $\pm$ 0.8 & 92.6 $\pm$ 0.3\\
        
        \hline
        Random attack ($\beta = 0.5$) & 68.5 $\pm$ 1.2   & 73.1 $\pm$ 1.1  & 71.2 $\pm$ 1.1 &  85.3 $\pm$ 1.1  & 89.8 $\pm$ 1.2 & 86.7 $\pm$ 1.1 \\
        Random attack ($\beta = 1.0$) & 60.1 $\pm$ 1.7   & 65.8 $\pm$ 1.4  & 62.3 $\pm$ 1.3 & 69.9 $\pm$ 1.3  & 81.3 $\pm$ 1.6 & 73.2 $\pm$ 0.9 \\
        
        \hline
        Gradient-based ($\Delta = 0.15$) & 66.1 $\pm$ 2.4 & 71.1 $\pm$ 1.4 & 67.3 $\pm$ 1.6  & 71.3 $\pm$ 1.1  & 79.6 $\pm$ 1.2 & 74.1 $\pm$ 0.8 \\
    
        \toprule
        
        
        \end{tabular}

\end{table*}

==> Tables/structural_perturbations.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t] 
\centering
\caption{Classification accuracy ($\pm$ standard deviation) of the models on different benchmark node classification dataset before (clean) and after the structural attacks application. The higher the accuracy (in \%) the better the model.}
\label{tab:structural_perturbations}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{0.10\textwidth}p{0.10\textwidth}cccccc@{}}
\toprule
Attack                   & \multicolumn{1}{c}{Model} & GCN        & GNN-Jaccard & RGCN           & GNN-SVD             & GNNGuard   & GCORN               \\ \midrule
\multirow{3}{*}{Mettack} & Cora                      & 71.4 $\pm$ 1.4 & 74.3 $\pm$ 1.6  & 62.7 $\pm$ 1.6          & 62.7 $\pm$ 1.6          & 74.4 $\pm$ 0.7 & \textbf{75.0 $\pm$ 1.8} \\
                         & CiteSeer                  & 63.5 $\pm$ 1.3 & 66.8 $\pm$ 1.2  & 65.4 $\pm$ 1.4          & 65.4 $\pm$ 1.4          & 66.8 $\pm$ 1.2 & \textbf{68.4 $\pm$ 1.6} \\
                         & PubMed                    & 73.3 $\pm$ 0.4 & 74.3 $\pm$ 1.2  & 73.0 $\pm$ 2.4          & \textbf{75.3 $\pm$ 1.5} & 75.1 $\pm$ 1.8 & 74.8 $\pm$ 2.4          \\ \midrule
\multirow{3}{*}{PGD}     & Cora                      & 71.7 $\pm$ 1.9 & 73.5 $\pm$ 0.6  & 73.1 $\pm$ 1.7          & 72.6 $\pm$ 1.2          & 73.8 $\pm$ 1.4 & \textbf{75.3 $\pm$ 1.6} \\
                         & CiteSeer                  & 62.3 $\pm$ 0.6 & 64.5 $\pm$ 0.4  & 57.7 $\pm$ 1.3          & 63.0 $\pm$ 0.9          & 64.8 $\pm$ 0.8 & \textbf{65.9 $\pm$ 0.6} \\
                         & PubMed                    & 63.0 $\pm$ 3.1 & 62.9 $\pm$ 1.4  & \textbf{63.3 $\pm$ 3.1} & 62.7 $\pm$ 1.8          & 63.1 $\pm$ 2.8 & 62.8 $\pm$ 2.6          \\ \bottomrule
\multirow{3}{*}{DICE}    & Cora                       & \multicolumn{1}{c}{67.4 $\pm$ 1.6} & 71.6 $\pm$ 0.7 & 69.7 $\pm$ 1.3                           & 65.4 $\pm$ 1.5                           & 72.6 $\pm$ 1.1          & \textbf{73.8 $\pm$ 1.4}                  \\
                         & CiteSeer                   & \multicolumn{1}{c}{59.1 $\pm$ 0.8} & 62.7 $\pm$ 1.1 & 60.8 $\pm$ 0.7                           & 60.1 $\pm$ 1.2                           & 63.9 $\pm$ 0.8          & \textbf{65.4 $\pm$ 1.8}                  \\
                         & PubMed                     & \multicolumn{1}{c}{70.8 $\pm$ 1.2} & 71.8 $\pm$ 1.3 & 71.5 $\pm$ 0.9                           & 74.3 $\pm$ 2.1                           & \textbf{74.9 $\pm$ 1.2} & 71.2 $\pm$ 1.3                           \\ \hline
\end{tabular}%
                         
}

\end{table}



==> chapters/limitations.tex <==
A clear limination of this work is that it was produced with academic computational resources as opposed to the computational resources available in industry. Our limited resources did not allow us to explore datasets, in which the different classes were sufficiently represented for our proposed graph construction to demonstrate its full potential. 

Another limitation is the increased memory cost of the \textit{DGoW} graph construction and consequently the \textit{DGoW-GNN} as compared to the more traditional graph constructions. The  number of nodes in \textit{DGoW} is larger the the number of nodes in \textit{MGoW}. If there are sufficiently many training sentences per class, then we believe this additional cost to be offset by the greater separateness of the classes in this informative graph.  




==> chapters/problem_formulation.tex <==
First of all, let us introduce the task of text classification. Given a set of training sentences  $\mathcal{S}^{train} = \{s^{train}_1, \ldots, s^{train}_N\}$ and theirs corresponding labels $\mathcal{Y}_{train} = \{y^{train}_1, \ldots, y^{train}_N\}$ , the goal is to train a model to predict $\mathcal{Y}_{train}$  and generalize it for the remaining unlabeled test sentences $\mathcal{S}^{test} = \{s^{test}_1, \ldots, s^{test}_M\}$.


Each training or test sentence $s$ is a sequence of words $s = [w^{(s)}_1,w^{(s)}_2,\ldots, w^{(s)}_{L(s)}]$ where $L(s)$ is the length of $s$. The number of words in a sentence depends on the data processing used for the dataset. The label of a sentence belongs necessarily to set of $P$ possible values : $\forall i, ~~y_i \in \{y_1,\ldots,y_P\}$.


